Boosting Differentiable Causal Discovery via Adaptive Sample Reweighting

Under stringent model type and variable distribution assumptions, differentiable score-based causal discovery methods learn a directed acyclic graph (DAG) from observational data by evaluating candidate graphs over an average score function. Despite great success in low-dimensional linear systems, it has been observed that these approaches overly exploit easier-to-fit samples, thus inevitably learning spurious edges. Worse still, inherent mostly in these methods the common homogeneity assumption can be easily violated, due to the widespread existence of heterogeneous data in the real world, resulting in performance vulnerability when noise distributions vary. We propose a simple yet effective model-agnostic framework to boost causal discovery performance by dynamically learning the adaptive weights for the Reweighted Score function, ReScore for short, where the weights tailor quantitatively to the importance degree of each sample. Intuitively, we leverage the bilevel optimization scheme to \wx{alternately train a standard DAG learner and reweight samples -- that is, upweight the samples the learner fails to fit and downweight the samples that the learner easily extracts the spurious information from. Extensive experiments on both synthetic and real-world datasets are carried out to validate the effectiveness of ReScore. We observe consistent and significant boosts in structure learning performance. Furthermore, we visualize that ReScore concurrently mitigates the influence of spurious edges and generalizes to heterogeneous data. Finally, we perform the theoretical analysis to guarantee the structure identifiability and the weight adaptive properties of ReScore in linear systems. Our codes are available at https://github.com/anzhang314/ReScore.

==> Backup/0-abstract.tex <==
\begin{abstract}
% Score-based causal discovery methods learn directed acyclic graphs from observation data by evaluating the candidate graphs with an averaged score function under stringent assumptions of model type and variable distribution.
Under stringent model type and variable distribution assumptions, score-based causal discovery methods learn the directed acyclic graph (DAG) from observational data by evaluating candidate graphs over an averaged score function.
Despite the great success in low-dimensional linear systems, it has been observed that these approaches overly exploits easier-to-fit samples, thus inevitably learning spurious edges.
Worse still, the common homogeneity assumption of most causal discovery methods can be easily violated due to the widespread existence of heterogeneous data in the real world, resulting in performance vulnerability when noise distributions vary. 
% Worse still, the widespread existence of heterogeneous data in the real world makes it easy to violate the common homogeneity assumption of most causal discovery methods, resulting in performance vulnerability when noise distributions vary. 
We propose a simple yet effective model-agnostic framework to boost causal discovery performance by dynamically learning the adaptive weights for the \textbf{Re}weighted \textbf{Score} function, \textbf{ReScore} for short, where the learned weights tailors quantitatively to the important degree of each samples.
Intuitively, we leverage the bilevel optimization scheme to \za{alternatingly} train a standard DAG learner first, then upweight the samples that the DAG learner fails to fit well and downweight the samples that the DAG learner easily extracts the causation information from.
Extensive experiments on both synthetic and real-world datasets are carried out to validate the effectiveness of ReScore.
We observe consistent and significant boosts in structure learning performance. 
We further visualize that ReScore concurrently mitigates the influence of spurious edges and generalizes to heterogeneous data.
Finally, we perform theoretical analysis to guarantee the structure identifiability and the weight adaptive properties of ReScore.
% We investigate a consistent and significant boosts in structure learning performance of ReScore, then further visualize that it concurrently mitigates the influence of spurious edges and generalizes to heterogeneous data.
% The theoretical guarantee of structure identifiability and weights adaptive property of ReScore are studied. 
% Extensive experimental results on both synthetic and real world datasets verify our analysis and demonstrate the effectiveness of ReScore.
Our codes are available at \url{https://anonymous.4open.science/r/ReScore-7631}.
\end{abstract}

==> Backup/1-introduction-new.tex <==

\section{Introduction}
Learning causal structure from purely observational data (\ie causal discovery) is a fundamental but daunting task \citep{NP-hard, Alzheimer}.
It strives to identify causal relationships between variables and encode the conditional independence as a directed acyclic graph (DAG).
Differentiable score-based optimization is a crucial enabler of causal discovery \citep{21survey}. 
Specifically, it is formulated as a continuous constraint optimization problem by minimizing the average score function and a smooth acyclicity constraint.
To ensure the structure is fully or partially identifiable (see Section \ref{sec:preliminary}), researchers impose stringent restrictions on model parametric family (\eg linear, additive) and common assumptions of variable distributions (\eg data homogeneity) \citep{ANM, MCSL}.
Following this scheme, recent follow-on studies \citep{SAM, GAE, RL-BIC, CAREFL, NoCurl} extend the formulation to general nonlinear problems by utilizing a variety of deep learning models.

However, upon careful inspections, we spot and justify two unsatisfactory behaviors of the current differentiable score-based methods:
\begin{itemize}[leftmargin=*]
    \item \wx{Differentiable} score-based causal discovery is error-prone to learning spurious edges or reverse causal directions between variables, which derails the structure learning accuracy \citep{DARING,convergence}.
    We substantiate our claim with an illustrative example as shown in Figure \ref{fig:motivation}.
    We find that even the fundamental structure, \ie chain, in a linear system, is easily misidentified by the state-of-the-art method, NOTEARS \citep{NOTEARS}.
    \item Despite being appealing in synthetic data, differentiable score-based methods suffer from severe performance degradation when encountering heterogeneous data \citep{CD-NOD,TVCM}.
    Considering Figure \ref{fig:motivation} again, NOTEARS is susceptible to learning redundant causations when the distributions of noise variables vary.
\end{itemize}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Motivation_Example.pdf}
    \vspace{-15pt}
    \caption{A simple example of basic chain structure that NOTEARS would learn spurious edges while ReScore can help to mitigate the bad influence.}
    \label{fig:motivation}
    \vspace{-5pt}
\end{figure*}

Taking a closer look at this dominant scheme (\ie optimizing the DAG learner via an average score function under strict assumptions), we ascribe these undesirable behaviors to its inherent limitations:
\begin{itemize}[leftmargin=*]
    \item The \wx{collected} datasets naturally include an overwhelming number of easy samples and a small number of informative samples that might contain crucial causation information \citep{hard_example_mining}.
    Averagely scoring the observational samples deprives the discovery process of differentiating sample importance, thus easy samples dominate the learning of DAG.
    As a result, prevailing score-based techniques fail to learn true causal relationship but instead yield the easier-to-fit spurious edges.
    % Intuitively, the average scoring assigns more weights to the majority groups of easy samples and less weights to the minority groups of hard samples.
    \item Noise distribution shifts are inevitable and common in real-world training, as the observations are typically collected at different periods, environments, locations, and so forth \citep{IRM}.
    As a result, the strong assumption of noise homogeneity for differentiable DAG learner is easily violated in real-world data \citep{CausalInference}. 
    A line of works \citep{MC&IB, DICD} dedicated to heterogeneous data can successfully address this issue.
    However, they often require explicit domain annotations (\ie ideal partition according to heterogeneity underlying the data) for each sample, which are prohibitively expensive and hard to obtain \citep{EIIL}, thus further limiting their applicability.
    
\end{itemize}

To reshape the optimization scheme and resolve these limitations, we propose to adaptively reweight the samples, which de facto concurrently mitigates the influence of spurious edges and generalizes to heterogeneous data.
The core idea is to discover and upweight a set of less-fitted samples that offer additional insight \wx{into depicting} the causal edges, compared to the samples that can be easily fitted via the spurious edges.
Focusing more on the less-fitted samples enables the DAG learner to effectively generalize to heterogeneous data, since in real-world scenarios, such samples typically come from disadvantaged domains.
However, due to the difficulty of accessing domain annotations, distinguishing such disadvantaged but informative samples and adaptively assigning their weights are challenging.
%In real-world scenarios, such less-fitted samples are mostly from the disadvantaged domains, hence focusing more on them allows the DAG learner to better generalize to heterogeneous data.
%Although, distinguishing such disadvantaged but informative samples is challenging, since the annotations of domains are expensive and difficult to obtain.

\wx{Towards this end, we present a simple yet effective model-agnostic optimization framework, coined \textbf{ReScore}, which automatically learns to reweight the samples and optimize the DAG learner, without any knowledge of domain annotations.
Specifically, we frame the adaptive weights learning and the DAG learning as a bilevel optimization problem:}

With the idea of adaptive sample reweighting, we present a simple yet effective model-agnostic optimization framework for DAG learner, coined \textbf{ReScore}, which alleviates the overfitting issue of easier-to-fit spurious edges.
On the other hand, ReScore tackles heterogeneous data without knowing the domain annotation in advance by automatically learning the instance-wise adaptive weights.
More precisely, we reformulate the adaptive weights learning as a bilevel optimization problem. 
The general model-agnostic bilevel scheme is designed below:
\begin{itemize}[leftmargin=*]
    \item In the inner loop, the DAG learner is evaluated by the reweighted score function to quantify the reliance on easier-to-fit samples and optimize the adaptive weights to achieve the worst-case.
    % 要写这个worst-case吗？会不会让人难以理解。
    \item In the outer loop, any score-based causal discovery method can be deployed to obtain the optimal DAG learner on weighted observational data where the weights are determined by the inner loop.
\end{itemize}
The inner loop and outer loop are iteratively trained. 
Benefiting from this optimization scheme, our ReScore has three desirable properties. 
First, ReScore is a model-agnostic technique that is flexible enough to easily adapt to any score-based causal discovery method. 
Moreover, we theoretically reveal that the structure identifiability is inherited by ReScore from the original causal discovery method (\cf Theorem \ref{thm:Identifiabilitytheorem}).
Second, ReScore jointly lightens the negative effect of spurious edge learning and performance drop in heterogeneous data by auto-learnable adaptive weights.
Theoretical analysis of adaptive properties for weights is provided in Section \ref{sec:adaptive} (\cf Theorem \ref{ReScoretheorem}).
Third, our proposed ReScore strengthens the existing causal discovery methods by a large margin. 
Surprisingly, ReScore performs competitively or even outperforms CD-NOD \citep{CD-NOD} and DICD \citep{DICD}, which require domain annotation, on heterogeneous synthetic data (\cf Section \ref{sec:exp_heterogeneous}).


==> Backup/1-introduction.tex <==
\section{Introduction}
% 1. Background of causal structure learning: Identifiability, Scalability; 

Learning causal structure from purely observational data is a fundamental but daunting task in machine learning \citep{NP-hard}, owing mainly to structural identifiability issues and the intractable combinatorial nature of acyclic space.  
To address the latter scalability difficulty, \cite{NOTEARS} reformulates the combinatorial problem as a differentiable score-based optimization problem by leveraging an algebraic characterization of acyclicity in the linear system.
Subsequent works extend the formulation to tackle general nonlinear problems by utilizing a variety of deep learning models and score functions \citep{SAM, GAE, DAG-GNN, RL-BIC, DARING}. 

Despite the unprecedented proliferation of literature and great success in linear case, differentiable score-based causal discovery methods suffer from severe performance degradation in nonlinear systems, especially when encounter heterogeneous data \citep{CD-NOD,TVCM}.
However, nonlinear and heterogeneous data are inevitable and common in real-world training, as complex causal relationship and distribution shift ubiquitously exists in data.
We attribute the performance decline of differentiable causal discovery methods to optimizing the average score loss.
The collecting datasets naturally contain an overwhelming number of easy samples and a small number of informative samples that might contain crucial causation information.
Structural learning models trained by average score function tend to relying on tremendous easy observations while ignoring the informative observations.
As a result, prevailing score-based causal discovery techniques fail to learn true causal relationship but instead exploit the easier-to-fit spurious edges, leading to poor performance on nonlinear and heterogeneous data.



% Our main purpose is to find an automatic selecting and effective reweighting of the observations so that the score-based causal discovery on the weighted data leads to superior performance.
% The identifiability property is inherent and the poor performance on heterogeneous data is naturally addressed.
% DAG learning models trained by average score function can fail to learn true causal relationship but instead exploit the easier-to-fit spurious edges, leading to poor performance on 

==> Backup/2-preliminary.tex <==

\section{Preliminary of Causal Discovery} \label{sec:preliminary}

Prevailing causal discovery approaches roughly fall into two reasearch lines, namely, constraint-based methods and score-based methods \citep{16survey,19survey}.
Constraint-based methods determine up to the Markov equivalence class of causal graphs according to conditional independent tests under certain assumptions \citep{latent_variable, PC, FCI, CAM}.
Score-based methods, on the other hand, evaluate the candidate graphs with a predefined score function and search over the space of directed acyclic graphs for the optimal graph \citep{21survey, NOFEARS}.
Here we focus on score-based causal discovery methods.

\textbf{Task Formulation.} 
Causal discovery problem aims to infer the Structural Causal Model (SCM) from observational data that best describe the data generating procedure.
Let $\rmX \in \gR^{n\times d}$ denote a data matrix consisting of n independent and identically distributed (i.i.d) random vectors $X =(X_1, \dots, X_d) \in \gR^d$.
A SCM $(P_X, \gG)$ encodes a causal directed acyclic graph (DAG) $\gG =(V(\gG),E(\gG))$ and a structural equation model, revealing the data generating process.
Specifically, the joint distribution $P_X$ over $X$ is Markov \wrt the DAG $\gG$, which factors the probability density function of $P_X$ as $p(x)= \prod_{i=1}^d P(x_i|x_{pa(i)})$, where $pa(i) = \{j \in V(\gG): X_j \rightarrow X_i \in E(\gG)\}$ refers the set of parents of $X_i$ in $\gG$ and $P(x_i|x_{pa(i)})$ denotes the conditional probability density function of variable $X_i$ given $X_{pa(i)}$. 
A structural equation model is defined as a collection of $d$ structural equations:
\begin{gather}\label{eq:SEM}
    X_i = f_i(X_{pa(i)},N_i), \quad i = 1,\dots,d
\end{gather}
where $f_i:\gR^{|X_{pa(i)}|} \rightarrow \gR $ can be any linear or nonlinear function and $N = (N_1,\dots,N_d)$ are jointly independent noise variables.

\textbf{Identifiability Issue.} 
In general, without further assumption on the structural equation model (\ie \eqref{eq:SEM}), it is not possible to infer $\gG$ by utilizing only observational data from $P_X$.
This arises identifiability issue in causal discovery. 
That is, whether a DAG $\gG$ can be uniquely identified.
More formally, given a set of assumptions on the structural equation model, its DAG $\gG$ is said to be identifiable over $P_X$, if no other structural equation model can encode the same distribution $P_X$ with a variant DAG under the same assumptions.
To guarantee the identifiability, most researchers restrict the form of the structural equations to be additive \wrt to noise, \ie additive noise models (ANM). 
Assuming ANM, as long as the structural equations are linear with non-Gaussian errors \citep{LiNGAM, Linear_nonGaussian}, linear Gaussian model with equal noise variances \citep{Linear_Gaussian_equal_noise}, or nonlinear structural equation model with mild conditions \citep{Nonlinear, Post_nonlinear, ANM},
then the DAG $\gG$ is identifiable.


\textbf{Score-based Causal Discovery.} 
With a slight abuse of notation, $\gG$ refers to a directed graph in the rest of the paper. The general formulation of conventional score-based causal discovery could be written as a combinatorial optimization problem:
\begin{align}\label{eq:score-comb}
    \min_{\gG} \quad & S(\gG;\rmX) = \Ls(\gG;\rmX) + \mathcal{R}_{sparse}(\gG) \nonumber\\
   \textrm{s.t.} \quad & \gG \in DAG
\end{align}
where the score function $S(\gG;\rmX)$ composes two terms - goodness-of-fit measure $\Ls(\gG;\rmX) = \frac{1}{n}\sum_{i=1}^{n}\Ls(\ervx_i, f(\ervx_i))$ and a sparsity regularization term $\mathcal{R}_{sparse}(\gG)$.
$\Ls(\ervx_i, f(\ervx_i))$ represents the fitting loss of observation $\ervx_i$ and $\mathcal{R}_{sparse}(\gG)$ encourages fewer edges in $\gG$.
The acyclicity constraint $\gG \in DAG$ is a challenge constraint.
In literature, there are various choices of search procedure for solving \eqref{eq:score-comb}, such as greedy search \citep{GES, GreedySearch}, hill-climbing \citep{hill_climbing, maxmin_hill-climbing}, dynamic programming \citep{DynamicProgram1, DynamicProgram2}, A* \citep{A}, and integer linear programming \citep{integer_prog1, integer_prog2}.

To fundamentally avoid combinatorial constraint $\gG \in DAG$, \cite{NOTEARS} recasts causal structural learning into a continuous constrained optimization problem
\begin{gather*}
    \min_{\gG} \, S(\gG;\rmX) \quad \textrm{s.t.} \,\, h(\gG) = 0
\end{gather*}
where $h(\gG) = 0$ is a differentiable equality DAG constraint. 
Suppose $\gA(\gG) \in \{0,1\}^{d\times d}$ defines the adjacent matrix of DAG $\gG$, such that $[\gA(\gG)]_{ij} =1 \Longleftrightarrow X_j \rightarrow X_i \in E(\gG)$.
Note that, there are various alternatives of $h(\gG)$ in the literature that incorporate different characterizations of DAGness, such as $h(\gG) = \Tr(e^{\gA \odot \gA})-d$, $h(\gG) = \Tr[(I+\alpha \gA\odot\gA)^d]-d$, and others \citep{NOFEARS, CASTLE, DAGMA}.

The unconstraint optimization problem is further formulated by using augmented Lagrangian method, which is denoted as
\begin{gather} \label{eq:score-cont}
    \min_{\gG} \, S(\gG;\rmX) + \mathcal{P}_{DAG}(\gG)
\end{gather}
where $\mathcal{P}_{DAG}(\gG) = \lambda h(\gG)$ is a penalty term enforcing DAGness on $\gG$.


There are plenty of possibilities to deﬁne the score function $S(\gG;\rmX)$, such as penalized Least-squares loss \citep{NOTEARS-MLP, NOTEARS, GAE}, Evidence Lower Bound (ELBO) \citep{DAG-GNN}, log-likelihood with complexity regularizers \citep{SAM}, penalized maximum likelihood estimator \citep{l0-penalized, GOLEM}, Maximum Mean Discrepancy (MMD) \citep{CGNN}, Bayesian Information Criterion (BIC) \citep{BIC, RL-BIC}, Bayesian Dirichlet equivalence uniform (BDeu) score \citep{BDe(u)}, Bayesian Gaussian equivalent (BGe) score \citep{BGe} and others \citep{GSF,KGV_score,Spearman_correlation}.

==> Backup/3-methodology.tex <==

\section{Methodology of ReScore}
On the basis of differentiable score-based causal discovery methods, we first devise our ReScore and then present its desirable properties.

\subsection{Bilevel Formulation of ReScore}
\wx{Aiming to learn the causal structure accurately in practical scenarios, we focus on the observational data that is heterogeneous and contains a large proportion of easy samples.
Standard differentiable score-based causal discovery methods apply the average score function on all samples equally, which inherently rely on easy samples to obtain high average goodness-of-fit.
As a result, the DAG learner is error-prone to constructing easier-to-fit spurious edges based on the easy samples, while ignoring the causal relationship information maintained in hard samples.
Assuming the oracle importance of each sample is known at hand, we can assign distinct weights to different samples and formulate the reweighted score function $S_\ervw(\gG;\rmX)$, instead of the average score function:}
\begin{align} \label{eq:score-weighted}
     S_\ervw(\gG;\rmX) = \Ls_\ervw(\gG;\rmX) + \lambda\mathcal{R}_{sparse}(\gG)  = \sum_{i=1}^{n} w_i l(\Mat{x}_i, f(\Mat{x}_i)) + \lambda\mathcal{R}_{sparse}(\gG),
\end{align}
where $\Mat{w} = (w_1,\dots,w_n)$ is a sample reweighting vector with length $n$, \wx{where $w_i$ indicates the importance of the $i$-th observed sample $\Mat{x}_{i}$.}


\wx{However, the oracle sample importance is usually unavailable in real-world scenarios.} The problem, hence, comes to how to automatically learn appropriate the sample reweighting vector $\Mat{w}$.
\wx{Intuitively, samples easily fitted with spurious edges should contribute less to the DAG learning, while samples that do not hold spurious edges but contain critical information about causal edges should be more importance.
We therefore use a simple heuristic of downweighting the easier-to-fit but less informative samples, and upweighting the less-fitted but more informative samples.
This inspires us to learn to allocate weights adaptively, with the aim of maximizing the influence of less-fitted samples and failing the DAG learner.
Formally, we cast the overall framework of reweighting samples to boost causal discovery as the following bilevel optimization problem:}
\czb{\begin{align} \label{maxweight}
    \min_{\Set{G}}~& S_{\ervw^*}(\gG;\rmX) + \mathcal{P}_{DAG}(\gG), \nonumber\\
    \textrm{s.t.}~& \Mat{w}^* \in \argmax_{\Mat{w} \in \sC(\tau)} \, S_{\ervw}(\gG;\rmX), 
\end{align}
where $ \sC(\tau) := \{\Mat{w}: 0 < \frac{\tau}{n} \leq w_1, \dots, w_n \leq \frac{1}{\tau n}, \sum_{i=1}^{n} w_i = 1\}$} for the \wx{cutoff threshold $ \tau \in (0, 1) $.} 
The deviation of the weight distribution from the uniform distribution is bound by the hyperparameter $\tau$.
\wx{Clearly, \Eqref{maxweight} consists of two objectives, where the inner-level objective (\ie optimize $\Mat{w}$ by maximizing the reweighted score function) is nested within the outer-level objective (\ie optimize $\Set{G}$ by minimizing the differentiable score-based loss).
Solving the outer-level problem should be subject to the optimal value of the inner-level problem.}
% The outer and inner objectives in this case can be any reweighted score function $S_{\ervw}(\gG;\rmX)$ derived from the existing score functions $S(\Set{G};\Mat{X})$ outlined in Section \ref{sec:preliminary}.

\wx{Now we introduce how to solve this bilevel optimization problem.
In the inner loop, we first fix the DAG learner which evaluates the error of each observed sample $\Mat{x}_{i}$, $\forall i\in\{1,\cdots,n\}$, and then maximize the reweighted score function to learn the weight $w_i^*$ correspondingly.
In the outer loop, upon the reweighted observations whose weights are determined in the inner loop, we minimize the reweighted score function to optimize the DAG learner.
By alternately training the inner and outer loops, the importance of each sample is adaptively estimated based on the DAG learner's error, and in turn gradually guides the DAG learner to perform better on the informative samples.
Overall, the procedure of training ReScore is outlined in Algorithm \ref{alg:ReScore}.
}

Furthermore, our ReScore has the following desirable advantages:
\begin{itemize}[leftmargin=*]
    \item As shown in Section \ref{sec:identifiability}, under mild conditions, our ReScore inherits the identifiability property of the original score-based causal discovery method.
    \item ReScore is able to automatically select the more informative samples and assign adaptive weights to each observation through bilevel optimization, which is consistent with our theoretical analysis in Section \ref{sec:adaptive} and empirical results in Section \ref{sec:exp_heterogeneous}.
    \item ReScore is widely applicable to various types of data and models. In other words, ReScore is model-agnostic and can effectively handle heterogeneous data without knowing the domain annotation in advance. Detailed ReScore performance can be found in Section \ref{sec:experiments}.
\end{itemize}

\subsection{Theoretical Analysis on Identifiability} \label{sec:identifiability}
Graph identifiability issues are the primary challenges hindering the development of structure learning.
As an optimization framework, the capacity of ReScore to ensure graph identifiability while substantially boosting the performance of the score-based DAG learner is the most desired property.
We develop Theorem \ref{thm:Identifiabilitytheorem} that guarantees the identifiability of the DAG using ReScore.

Recall that to render a DAG theoretically identifiable, three standard steps are necessary \citep{NOTEARS-MLP, ANM, convergence}:
\za{Initially, the particular restricted family of functions and data distributions of SEM in \Eqref{eq:SEM} are assumed.}
The second step is to theoretically prove the SEM's identifiability.
Thirdly, developing an optimization algorithm with a predefined score function and showing the learned DAG asymptotically converges to the ground-truth DAG.
Clearly, ReScore naturally inherits the original identifiability of a specific SEM as stated in Section \ref{sec:preliminary}.
The key concern arising is whether the DAG learned by our new optimization framework under reweighted score function $S_\ervw(\gG;\rmX)$ can asymptotically converge to the ground-truth DAG.
Fortunately, \czb{similar weights have common used in unbalanced classification problems. One can also treat the ReScore procedure as a resampling step in bootstrapping with a sequence of weights. In addition, }
the following theorem demonstrates that, by guaranteeing the equivalence of optimization problems (\ref{eq:score-comb}) and (\ref{maxweight}) in linear systems, the bounded weights will not affect the consistency results in identifiability analysis.
See detailed proof in Appendix \ref{sec:proof1}.

% Existing papers resolve the issue into five steps: 1) Give a specific model for SEM; 2) Show the identifiability for the given model; 3) Select a loss function for optimization; 4) Develop an algorithm for learning that model; 5) Prove the learned model converge to the ground truth asymptotically. 
% Clearly, in this paper, we always inherit the previous models, so that the proof of identifiability in step 2) follows naturally. The key improvement for the ReScore method is the ReScore function defined in \Eqref{eq:score-weighted}, which influence the loss function and subsequent steps (steps 3 ~ 5 ). The following theorem reveals that the reweight will not influence the consistency results in identifiability analysis. 

\begin{restatable}{theorem}{Identifiability} \label{thm:Identifiabilitytheorem}
\czb{Suppose the SEM in \Eqref{eq:SEM} is linear and the size of observational data $\Mat{X}$ is $n$. As the data size increase, i.e. $ n \to \infty $, 
\begin{align*}
    \argmin_{\gG} \big\{ S_\Mat{w}(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} - \argmin_{\gG} \big\{ S(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} \xrightarrow[]{a.s.} \bf{0}
\end{align*}}
under the following cases.
% The optimization problem $ \min_{\gG} \big\{ S(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} $ is equivalent to $ \min_{\gG} \big\{ S_\ervw(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} $ asymptotically in the following cases. 
%Let $\Mat{w} \in \sC \czb{:= \{\Mat{w}: 0 < \frac{\tau}{n} \leq w_1, \dots, w_n \leq \frac{1}{\tau n}, \sum_{i=1}^{n} w_i = 1\}}$ for some small $ \tau > 0 $ and the SEM in \Eqref{eq:SEM} is linear. The optimization problem $ \min_{\gG} \big\{ S(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} $ is equivalent to $ \min_{\gG} \big\{ S_\ervw(\gG; \Mat{X}) + \mathcal{P}_{DAG}(\gG) \big\} $ asymptotically in the following cases. 
\begin{itemize}
    \item[a.] Using the least-squares loss $\Lapl(\Set{G};\Mat{X}) = \frac{1}{2n}\Vert \Mat{X} - f(\Mat{X}) \Vert_F^2$;
    \item[b.] Using the negative log-likelihood loss with standard Gaussian noise.
\end{itemize}
\end{restatable}

{\bf Remark:} The identifiability property of ReScore under two special but most common score functions, namely least-square loss and \czb{negative log-likelihood loss}, is proved in Theorem \ref{thm:Identifiabilitytheorem}.
% Only two special but most common cases are proved in this section, one is easy to derive similar results for other loss functions.
Similar conclusions can be easily derived for other loss functions, \czb{which are omitted as the length limit.}


\subsection{Oracle Property of Adaptive Weights} \label{sec:adaptive} 

Our ReScore suggests assigning varying degrees of importance to observational samples. 
The less-fitted samples are fundamentally more important than the easier-to-fit samples as they contain the causation information the DAG learner fails to extract.
That hard-to-learn causation information is the key to helping DAG learners mitigate the learning of spurious edges.
% The following theorem helps to illustrate the weights in our ReScore algorithm achieve our expectation.
The following theorem illustrates the adaptiveness property of ReScore, \ie instead of equally treating all the samples, ReScore tends to upweight the importance of informative and hard samples while downweighting the reliance on easier-to-fit samples.

\begin{restatable}{theorem}{AdaptiveProperty} \label{ReScoretheorem}
Suppose that in the optimization \za{phase}, the $i$-th observation has a larger error than the j-th observation in the sense that $l(\Mat{x}_i, f(\Mat{x}_i)) > l(\Mat{x}_j, f(\Mat{x}_j))$, where $i, j \in \{1, \dots, n\}$. Then, 
$$
w^*_i \czb{\geq} w^*_j,
$$
where $\Mat{w}^* = (w_1^*, \dots, w_n^*)$ is the optimal weights in \Eqref{maxweight}. \czb{The equality holds if and only if $ w^*_1 = w^*_2 = \frac{\tau}{n} $ or $ w^*_1 = w^*_2 = \frac{1}{\tau n} $. }
\end{restatable}

\czb{Please note that the errors used in this theorem are true values of a given model, which is not exactly same as the values in Algorithm \ref{alg:ReScore}.}  See detailed proof in Appendix \ref{sec:proof2}.
It is simple to infer that, following an inner loop for maximizing the reweighted score function $S_{\ervw}(\gG;\rmX)$, the observations are ranked by learned adaptive weights $\Mat{w}^*$.
In other words, one observation equipped with a higher weight will have a stronger impact on the subsequent outer loop to dominate the DAG learning.
% Thus, it is easy to derive that after an inner loop for maximizing score function $S_{w}(\gG;\rmX)$, the observations in data matrix $\rmX$ are ordered by their importance according to $\ervw^*$. In other words, one observation has more information when it has larger score, and it will contribute more in the next outer loop because of the larger weight. 
